Deep Generative Modeling for Protein Design

Deep learning approaches have produced substantial breakthroughs in fields such as image classification and natural language processing and are making rapid inroads in the area of protein design. Many generative models of proteins have been developed that encompass all known protein sequences, model specific protein families, or extrapolate the dynamics of individual proteins. Those generative models can learn protein representations that are often more informative of protein structure and function than hand-engineered features. Furthermore, they can be used to quickly propose millions of novel proteins that resemble the native counterparts in terms of expression level, stability, or other attributes. The protein design process can further be guided by discriminative oracles to select candidates with the highest probability of having the desired properties. In this review, we discuss five classes of generative models that have been most successful at modeling proteins and provide a framework for model guided protein design.

==> scratch.tex <==

Shanehsazzadeh et al. \cite{shanehsazzadehTransferLearningNecessary2020} noted that on many single protein stability and variant effect prediction tasks, simple linear regression performs surprisingly well and a convolutional neural network trained from scratch can outperform pretrained language-based models.
% Is Transfer Learning Necessary for Protein Landscape Prediction? \cite{shanehsazzadehTransferLearningNecessary2020}.

Using a one-hot representation of the amino acid sequence augmented with sequence log-likelihoods or pseudo log-likelihoods often leads produces better results than training using the model embeddings and without the amino acid sequence, especially in cases where training data are abundant \cite{hsuCombiningEvolutionaryAssaylabelled2021}. An augmented Potts model constructed from an MSA leads to higher performance than augmenting ESM-1b. However, Hsu et al. did not compare the augmented Potts model to augmenting deep learning models.

While transformers have led to breakthroughs in many NLP tasks, the practical applications of transformers trained on amino acid sequences have so far been limited. Rao et al. \cite{raoEvaluatingProteinTransfer2019} showed that protein representations generated using transformers are less

